Rate Loss in Quantum Channels with Classical State and Applications for Quantum Broadcast Channels

We consider the problem of \textit{rate loss} - a strict penalty suffered in achievable rates due to the lack of channel state information at the receiver (Rx) of a classical-quantum (CQ) channel. First, we identify non-commutative CQ channels and analytically prove a rate loss. Building on this, we next prove that coset-code-based strategies can strictly outperform conventional unstructured IID-code-based strategies for non-commutative 3-user CQ broadcast channels.

==> sty/LatexMacroDefinitions.tex <==
\def\naturals{\mathbb{N}}
\def\reals{\mathbb{R}}
\def\complex{\mathbb{C}}
\def\integers{\mathbb{Z}}
\def\fieldq{\mathcal{F}_{q}}
\def\Expectation{\mathbb{E}}

\newcommand{\msout}[1]{\text{\sout{\ensuremath{#1}}}}
% \newcommand{\comment}[1]{}

%================================
%==== COLORS =======
%================================

\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkmagenta}{rgb}{.5,0,.5}
\definecolor{darkblue}{rgb}{0,0,0.5}
% \definecolor{darkgray}{0.5,0.5,0.5}


%================================
%====\mathcal Letters =======
%================================

\def\CalA{\mathcal{A}}
\def\CalB{\mathcal{B}}
\def\CalC{\mathcal{C}}
\def\CalD{\mathcal{D}}
\def\CalE{\mathcal{E}}
\def\CalF{\mathcal{F}}
\def\CalG{\mathcal{G}}
\def\CalH{\mathcal{H}}
\def\CalI{\mathcal{I}}
\def\CalJ{\mathcal{J}}
\def\CalK{\mathcal{K}}
\def\CalL{\mathcal{L}}
\def\CalM{\mathcal{M}}
\def\CalN{\mathcal{N}}
\def\CalO{\mathcal{O}}
\def\CalP{\mathcal{P}}
\def\CalQ{\mathcal{Q}}
\def\CalR{\mathcal{R}}
\def\CalS{\mathcal{S}}
\def\CalT{\mathcal{T}}
\def\CalU{\mathcal{U}}
\def\CalV{\mathcal{V}}
\def\CalW{\mathcal{W}}
\def\CalX{\mathcal{X}}
\def\CalY{\mathcal{Y}}
\def\CalZ{\mathcal{Z}}



%================================
%=========UNDERLINES=============

\def\ulineA{\underline{A}}
\def\ulineB{\underline{B}}
\def\ulineC{\underline{C}}
\def\ulineD{\underline{D}}
\def\ulineE{\underline{E}}
\def\ulineF{\underline{F}}
\def\ulineG{\underline{G}}
\def\ulineH{\underline{H}}
\def\ulineI{\underline{I}}
\def\ulineJ{\underline{J}}
\def\ulineK{\underline{K}}
\def\ulineL{\underline{L}}
\def\ulineM{\underline{M}}
\def\ulineN{\underline{N}}
\def\ulineO{\underline{O}}
\def\ulineP{\underline{P}}
\def\ulineQ{\underline{Q}}
\def\ulineR{\underline{R}}
\def\ulineS{\underline{S}}
\def\ulineT{\underline{T}}
\def\ulineU{\underline{U}}
\def\ulineV{\underline{V}}
\def\ulineW{\underline{W}}
\def\ulineX{\underline{X}}
\def\ulineY{\underline{Y}}
\def\ulineZ{\underline{Z}}


\def\ulinea{\underline{a}}
\def\ulineb{\underline{b}}
\def\ulinec{\underline{c}}
\def\ulined{\underline{d}}
\def\ulinee{\underline{e}}
\def\ulinef{\underline{f}}
\def\ulineg{\underline{g}}
\def\ulineh{\underline{h}}
\def\ulinei{\underline{i}}
\def\ulinej{\underline{j}}
\def\ulinek{\underline{k}}
\def\ulinel{\underline{l}}
\def\ulinem{\underline{m}}
\def\ulinen{\underline{n}}
\def\ulineo{\underline{o}}
\def\ulinep{\underline{p}}
\def\ulineq{\underline{q}}
\def\uliner{\underline{r}}
\def\ulines{\underline{s}}
\def\ulinet{\underline{t}}
\def\ulineu{\underline{u}}
\def\ulinev{\underline{v}}
\def\ulinew{\underline{w}}
\def\ulinex{\underline{x}}
\def\uliney{\underline{y}}
\def\ulinez{\underline{z}}

\def\ulinePi{\underline{\Pi}}
\def\ulinepi{\underline{\pi}}

% \def\uline0{\underline{0}}


%================================
%=========UNDERLINES==GREEK======


\def\ulinetheta{\underline{\theta}}
\def\ulinemu{\underline{\mu}}
\def\ulinetau{\underline{\tau}}
%============================================
%=========HAT ON TOP - LOWERCASE=============

\def\hata{\hat{a}}
\def\hatb{\hat{b}}
\def\hatc{\hat{c}}
\def\hatd{\hat{d}}
\def\hate{\hat{e}}
\def\hatf{\hat{f}}
\def\hatg{\hat{g}}
\def\hath{\hat{h}}
\def\hati{\hat{i}}
\def\hatj{\hat{j}}
\def\hatk{\hat{k}}
\def\hatl{\hat{l}}
\def\hatm{\hat{m}}
\def\hatn{\hat{n}}
\def\hato{\hat{o}}
\def\hatp{\hat{p}}
\def\hatq{\hat{q}}
\def\hatr{\hat{r}}
\def\hats{\hat{s}}
\def\hatt{\hat{t}}
\def\hatu{\hat{u}}
\def\hatv{\hat{v}}
\def\hatw{\hat{w}}
\def\hatx{\hat{x}}
\def\haty{\hat{y}}
\def\hatz{\hat{z}}


%================================
%====\mathcal Letters =======
%================================

\def\CalA{\mathcal{A}}
\def\CalB{\mathcal{B}}
\def\CalC{\mathcal{C}}
\def\CalD{\mathcal{D}}
\def\CalE{\mathcal{E}}
\def\CalF{\mathcal{F}}
\def\CalG{\mathcal{G}}
\def\CalH{\mathcal{H}}
\def\CalI{\mathcal{I}}
\def\CalJ{\mathcal{J}}
\def\CalK{\mathcal{K}}
\def\CalL{\mathcal{L}}
\def\CalM{\mathcal{M}}
\def\CalN{\mathcal{N}}
\def\CalO{\mathcal{O}}
\def\CalP{\mathcal{P}}
\def\CalQ{\mathcal{Q}}
\def\CalR{\mathcal{R}}
\def\CalS{\mathcal{S}}
\def\CalT{\mathcal{T}}
\def\CalU{\mathcal{U}}
\def\CalV{\mathcal{V}}
\def\CalW{\mathcal{W}}
\def\CalX{\mathcal{X}}
\def\CalY{\mathcal{Y}}
\def\CalZ{\mathcal{Z}}


%============================================
%=========HAT ON TOP - UPPERCASE=============

\def\hatA{\hat{A}}
\def\hatB{\hat{B}}
\def\hatC{\hat{C}}
\def\hatD{\hat{D}}
\def\hatE{\hat{E}}
\def\hatF{\hat{F}}
\def\hatG{\hat{G}}
\def\hatH{\hat{H}}
\def\hatI{\hat{I}}
\def\hatJ{\hat{J}}
\def\hatK{\hat{K}}
\def\hatL{\hat{L}}
\def\hatM{\hat{M}}
\def\hatN{\hat{N}}
\def\hatO{\hat{O}}
\def\hatP{\hat{P}}
\def\hatQ{\hat{Q}}
\def\hatR{\hat{R}}
\def\hatS{\hat{S}}
\def\hatT{\hat{T}}
\def\hatU{\hat{U}}
\def\hatV{\hat{V}}
\def\hatW{\hat{W}}
\def\hatX{\hat{X}}
\def\hatY{\hat{Y}}
\def\hatZ{\hat{Z}}




\def\ulineCalA{\underline{\mathcal{A}}}
\def\ulineCalB{\underline{\mathcal{B}}}
\def\ulineCalC{\underline{\mathcal{C}}}
\def\ulineCalD{\underline{\mathcal{D}}}
\def\ulineCalE{\underline{\mathcal{E}}}
\def\ulineCalF{\underline{\mathcal{F}}}
\def\ulineCalG{\underline{\mathcal{G}}}
\def\ulineCalH{\underline{\mathcal{H}}}
\def\ulineCalI{\underline{\mathcal{I}}}
\def\ulineCalJ{\underline{\mathcal{J}}}
\def\ulineCalK{\underline{\mathcal{K}}}
\def\ulineCalL{\underline{\mathcal{L}}}
\def\ulineCalM{\underline{\mathcal{M}}}
\def\ulineCalN{\underline{\mathcal{N}}}
\def\ulineCalO{\underline{\mathcal{O}}}
\def\ulineCalP{\underline{\mathcal{P}}}
\def\ulineCalQ{\underline{\mathcal{Q}}}
\def\ulineCalR{\underline{\mathcal{R}}}
\def\ulineCalS{\underline{\mathcal{S}}}
\def\ulineCalT{\underline{\mathcal{T}}}
\def\ulineCalU{\underline{\mathcal{U}}}
\def\ulineCalV{\underline{\mathcal{V}}}
\def\ulineCalW{\underline{\mathcal{W}}}
\def\ulineCalX{\underline{\mathcal{X}}}
\def\ulineCalY{\underline{\mathcal{Y}}}
\def\ulineCalZ{\underline{\mathcal{Z}}}




%==========================================================
%=========UNDERLINE and HAT ON TOP - LOWERCASE=============

\def\ulinehata{\hat{\underline{a}}}
\def\ulinehatb{\hat{\underline{b}}}
\def\ulinehatc{\hat{\underline{c}}}
\def\ulinehatd{\hat{\underline{d}}}
\def\ulinehate{\hat{\underline{e}}}
\def\ulinehatf{\hat{\underline{f}}}
\def\ulinehatg{\hat{\underline{g}}}
\def\ulinehath{\hat{\underline{h}}}
\def\ulinehati{\hat{\underline{i}}}
\def\ulinehatj{\hat{\underline{j}}}
\def\ulinehatk{\hat{\underline{k}}}
\def\ulinehatl{\hat{\underline{l}}}
\def\ulinehatm{\hat{\underline{m}}}
\def\ulinehatn{\hat{\underline{n}}}
\def\ulinehato{\hat{\underline{o}}}
\def\ulinehatp{\hat{\underline{p}}}
\def\ulinehatq{\hat{\underline{q}}}
\def\ulinehatr{\hat{\underline{r}}}
\def\ulinehats{\hat{\underline{s}}}
\def\ulinehatt{\hat{\underline{t}}}
\def\ulinehatu{\hat{\underline{u}}}
\def\ulinehatv{\hat{\underline{v}}}
\def\ulinehatw{\hat{\underline{w}}}
\def\ulinehatx{\hat{\underline{x}}}
\def\ulinehaty{\hat{\underline{y}}}
\def\ulinehatz{\hat{\underline{z}}}


\def\noi{\noindent}
\def\parsec{\par\noindent}
\def\med{\medskip\parsec}

\def\lnn{\nonumber} %Used for the last line of an equtn array where we do not want a equation number to appear
\def\nnn{\nonumber\newline}
\def\nln{\newline}




\def\define{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}


\def\boldCalA{\boldsymbol{\mathcal{A}}}
\def\boldCalB{\boldsymbol{\mathcal{B}}}
\def\boldCalC{\boldsymbol{\mathcal{C}}}
\def\boldCalD{\boldsymbol{\mathcal{D}}}
\def\boldCalE{\boldsymbol{\mathcal{E}}}
\def\boldCalF{\boldsymbol{\mathcal{F}}}
\def\boldCalG{\boldsymbol{\mathcal{G}}}
\def\boldCalH{\boldsymbol{\mathcal{H}}}
\def\boldCalI{\boldsymbol{\mathcal{I}}}
\def\boldCalJ{\boldsymbol{\mathcal{J}}}
\def\boldCalK{\boldsymbol{\mathcal{K}}}
\def\boldCalL{\boldsymbol{\mathcal{L}}}
\def\boldCalM{\boldsymbol{\mathcal{M}}}
\def\boldCalN{\boldsymbol{\mathcal{N}}}
\def\boldCalO{\boldsymbol{\mathcal{O}}}
\def\boldCalP{\boldsymbol{\mathcal{P}}}
\def\boldCalQ{\boldsymbol{\mathcal{Q}}}
\def\boldCalR{\boldsymbol{\mathcal{R}}}
\def\boldCalS{\boldsymbol{\mathcal{S}}}
\def\boldCalT{\boldsymbol{\mathcal{T}}}
\def\boldCalU{\boldsymbol{\mathcal{U}}}
\def\boldCalV{\boldsymbol{\mathcal{V}}}
\def\boldCalW{\boldsymbol{\mathcal{W}}}
\def\boldCalX{\boldsymbol{\mathcal{X}}}
\def\boldCalY{\boldsymbol{\mathcal{Y}}}
\def\boldCalZ{\boldsymbol{\mathcal{Z}}}


\def\boldA{\boldsymbol{A}}
\def\boldB{\boldsymbol{B}}
\def\boldC{\boldsymbol{C}}
\def\boldD{\boldsymbol{D}}
\def\boldE{\boldsymbol{E}}
\def\boldF{\boldsymbol{F}}
\def\boldG{\boldsymbol{G}}
\def\boldH{\boldsymbol{H}}
\def\boldI{\boldsymbol{I}}
\def\boldJ{\boldsymbol{J}}
\def\boldK{\boldsymbol{K}}
\def\boldL{\boldsymbol{L}}
\def\boldM{\boldsymbol{M}}
\def\boldN{\boldsymbol{N}}
\def\boldO{\boldsymbol{O}}
\def\boldP{\boldsymbol{P}}
\def\boldQ{\boldsymbol{Q}}
\def\boldR{\boldsymbol{R}}
\def\boldS{\boldsymbol{S}}
\def\boldT{\boldsymbol{T}}
\def\boldU{\boldsymbol{U}}
\def\boldV{\boldsymbol{V}}
\def\boldW{\boldsymbol{W}}
\def\boldX{\boldsymbol{X}}
\def\boldY{\boldsymbol{Y}}
\def\boldZ{\boldsymbol{Z}}


\def\bolda{\boldsymbol{a}}
\def\boldb{\boldsymbol{b}}
\def\boldc{\boldsymbol{c}}
\def\boldd{\boldsymbol{d}}
\def\bolde{\boldsymbol{e}}
\def\boldf{\boldsymbol{f}}
\def\boldg{\boldsymbol{g}}
\def\boldh{\boldsymbol{h}}
\def\boldi{\boldsymbol{i}}
\def\boldj{\boldsymbol{j}}
\def\boldk{\boldsymbol{k}}
\def\boldl{\boldsymbol{l}}
\def\boldn{\boldsymbol{m}}
\def\boldo{\boldsymbol{n}}
\def\boldp{\boldsymbol{o}}
\def\boldP{\boldsymbol{p}}
\def\boldq{\boldsymbol{q}}
\def\boldr{\boldsymbol{r}}
\def\bolds{\boldsymbol{s}}
\def\boldt{\boldsymbol{t}}
\def\boldu{\boldsymbol{u}}
\def\boldv{\boldsymbol{v}}
\def\boldw{\boldsymbol{w}}
\def\boldx{\boldsymbol{x}}
\def\boldy{\boldsymbol{y}}
\def\boldz{\boldsymbol{z}}

%%%%%%%%%%%% 04Aug2024 : Why is the FOLLOWING here? Clean it up?
\def\boldd{\boldsymbol{d}}
\def\boldR{\boldsymbol{R}}
\def\boldm{\boldsymbol{m}}
\def\boldS{\boldsymbol{S}}
\def\bolds{\boldsymbol{s}}
\def\bolda{\boldsymbol{a}}
\def\boldb{\boldsymbol{b}}
\def\boldX{\boldsymbol{X}}
\def\boldx{\boldsymbol{x}}
\def\boldU{\boldsymbol{U}}
\def\boldu{\boldsymbol{u}}
\def\boldY{\boldsymbol{Y}}
\def\boldy{\boldsymbol{y}}
\def\boldV{\boldsymbol{V}}
\def\boldv{\boldsymbol{v}}
\def\boldZ{\boldsymbol{Z}}
\def\boldz{\boldsymbol{z}}
\def\boldA{\boldsymbol{A}}
\def\boldB{\boldsymbol{B}}
\def\boldG{\boldsymbol{G}}
\def\boldW{\boldsymbol{W}}
\def\boldw{\boldsymbol{w}}


%%%%%%%%%%%% 04Aug2024 : Why is the ABOVE here? Clean it up?



\def\boldlambda{\boldsymbol{\lambda}}
\def\boldvphi{\boldsymbol{\varphi}}
\def\boldrho{\boldsymbol{\rho}}
\def\boldbeta{\boldsymbol{\beta}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%Overline Characters%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\def\olinea{\overline{a}}
\def\olineb{\overline{b}}
\def\olinec{\overline{c}}
\def\olined{\overline{d}}
\def\olinee{\overline{e}}
\def\olinef{\overline{f}}
\def\olineg{\overline{g}}
\def\olineh{\overline{h}}
\def\olinei{\overline{i}}
\def\olinej{\overline{j}}
\def\olinek{\overline{k}}
\def\olinel{\overline{l}}
\def\olinem{\overline{m}}
\def\olinen{\overline{n}}
\def\olineo{\overline{o}}
\def\olinep{\overline{p}}
\def\olineq{\overline{q}}
\def\oliner{\overline{r}}
\def\olines{\overline{s}}
\def\olinet{\overline{t}}
\def\olineu{\overline{u}}
\def\olinev{\overline{v}}
\def\olinew{\overline{w}}
\def\olinex{\overline{x}}
\def\oliney{\overline{y}}
\def\olinez{\overline{z}}



\def\olineA{\overline{A}}
\def\olineB{\overline{B}}
\def\olineC{\overline{C}}
\def\olineD{\overline{D}}
\def\olineE{\overline{E}}
\def\olineF{\overline{F}}
\def\olineG{\overline{G}}
\def\olineH{\overline{H}}
\def\olineI{\overline{I}}
\def\olineJ{\overline{J}}
\def\olineK{\overline{K}}
\def\olineL{\overline{L}}
\def\olineM{\overline{M}}
\def\olineN{\overline{N}}
\def\olineO{\overline{O}}
\def\olineP{\overline{P}}
\def\olineQ{\overline{Q}}
\def\olineR{\overline{R}}
\def\olineS{\overline{S}}
\def\olineT{\overline{T}}
\def\olineU{\overline{U}}
\def\olineV{\overline{V}}
\def\olineW{\overline{W}}
\def\olineX{\overline{X}}
\def\olineY{\overline{Y}}
\def\olineZ{\overline{Z}}


\def\thetabar{\overline{\theta}}
\def\olDelta{\overline{\Delta}}
\def\olineDelta{\overline{\Delta}}




%================================
%====\mathscr Letters =======
%================================

\def\ScrA{\mathscr{A}}
\def\ScrB{\mathscr{B}}
\def\ScrC{\mathscr{C}}
\def\ScrD{\mathscr{D}}
\def\ScrE{\mathscr{E}}
\def\ScrF{\mathscr{F}}
\def\ScrG{\mathscr{G}}
\def\ScrH{\mathscr{H}}
\def\ScrI{\mathscr{I}}
\def\ScrJ{\mathscr{J}}
\def\ScrK{\mathscr{K}}
\def\ScrL{\mathscr{L}}
\def\ScrM{\mathscr{M}}
\def\ScrN{\mathscr{N}}
\def\ScrO{\mathscr{O}}
\def\ScrP{\mathscr{P}}
\def\ScrQ{\mathscr{Q}}
\def\ScrR{\mathscr{R}}
\def\ScrS{\mathscr{S}}
\def\ScrT{\mathscr{T}}
\def\ScrU{\mathscr{U}}
\def\ScrV{\mathscr{V}}
\def\ScrW{\mathscr{W}}
\def\ScrX{\mathscr{X}}
\def\ScrY{\mathscr{Y}}
\def\ScrZ{\mathscr{Z}}


%================================
%====\teletype Letters =======
%================================


\def\tta{\mathtt{a}}
\def\ttb{\mathtt{b}}
\def\ttc{\mathtt{c}}
\def\ttd{\mathtt{d}}
\def\tte{\mathtt{e}}
\def\ttf{\mathtt{f}}
\def\ttg{\mathtt{g}}
\def\tth{\mathtt{h}}
\def\tti{\mathtt{i}}
\def\ttj{\mathtt{j}}
\def\ttk{\mathtt{k}}
\def\ttl{\mathtt{l}}
\def\ttm{\mathtt{m}}
\def\ttn{\mathtt{n}}
\def\tto{\mathtt{o}}
\def\ttp{\mathtt{p}}
\def\ttq{\mathtt{q}}
\def\ttr{\mathtt{r}}
\def\tts{\mathtt{s}}
\def\ttt{\mathtt{t}}
\def\ttu{\mathtt{u}}
\def\ttv{\mathtt{v}}
\def\ttw{\mathtt{w}}
\def\ttx{\mathtt{x}}
\def\tty{\mathtt{y}}
\def\ttz{\mathtt{z}}

\def\ttA{\mathtt{A}}
\def\ttB{\mathtt{B}}
\def\ttC{\mathtt{C}}
\def\ttD{\mathtt{D}}
\def\ttE{\mathtt{E}}
\def\ttF{\mathtt{F}}
\def\ttG{\mathtt{G}}
\def\ttH{\mathtt{H}}
\def\ttI{\mathtt{I}}
\def\ttJ{\mathtt{J}}
\def\ttK{\mathtt{K}}
\def\ttL{\mathtt{L}}
\def\ttM{\mathtt{M}}
\def\ttN{\mathtt{N}}
\def\ttO{\mathtt{O}}
\def\ttP{\mathtt{P}}
\def\ttQ{\mathtt{Q}}
\def\ttR{\mathtt{R}}
\def\ttS{\mathtt{S}}
\def\ttT{\mathtt{T}}
\def\ttU{\mathtt{U}}
\def\ttV{\mathtt{V}}
\def\ttW{\mathtt{W}}
\def\ttX{\mathtt{X}}
\def\ttY{\mathtt{Y}}
\def\ttZ{\mathtt{Z}}


%================================
%====\mathsf Lowercase Letters =======
%================================

\def\sfa{\mathsf{a}}
\def\sfb{\mathsf{b}}
\def\sfc{\mathsf{c}}
\def\sfd{\mathsf{d}}
\def\sfe{\mathsf{e}}
\def\sff{\mathsf{f}}
\def\sfg{\mathsf{g}}
\def\sfh{\mathsf{h}}
\def\sfi{\mathsf{i}}
\def\sfj{\mathsf{j}}
\def\sfk{\mathsf{k}}
\def\sfl{\mathsf{l}}
\def\sfm{\mathsf{m}}
\def\sfn{\mathsf{n}}
\def\sfo{\mathsf{o}}
\def\sfp{\mathsf{p}}
\def\sfq{\mathsf{q}}
\def\sfr{\mathsf{r}}
\def\sfs{\mathsf{s}}
\def\sft{\mathsf{t}}
\def\sfu{\mathsf{u}}
\def\sfv{\mathsf{v}}
\def\sfw{\mathsf{w}}
\def\sfx{\mathsf{x}}
\def\sfy{\mathsf{y}}
\def\sfz{\mathsf{z}}

%================================
%====\mathsf Uppercase Letters =======
%================================

\def\sfA{\mathsf{A}}
\def\sfB{\mathsf{B}}
\def\sfC{\mathsf{C}}
\def\sfD{\mathsf{D}}
\def\sfE{\mathsf{E}}
\def\sfF{\mathsf{F}}
\def\sfG{\mathsf{G}}
\def\sfH{\mathsf{H}}
\def\sfI{\mathsf{I}}
\def\sfJ{\mathsf{J}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfM{\mathsf{M}}
\def\sfN{\mathsf{N}}
\def\sfO{\mathsf{O}}
\def\sfP{\mathsf{P}}
\def\sfQ{\mathsf{Q}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfU{\mathsf{U}}
\def\sfV{\mathsf{V}}
\def\sfW{\mathsf{W}}
\def\sfX{\mathsf{X}}
\def\sfY{\mathsf{Y}}
\def\sfZ{\mathsf{Z}}

%================================
%====\tilde at the top =======
%================================

\def\tildea{\tilde{a}}
\def\tildeb{\tilde{b}}
\def\tildec{\tilde{c}}
\def\tilded{\tilde{d}}
\def\tildee{\tilde{e}}
\def\tildef{\tilde{f}}
\def\tildeg{\tilde{g}}
\def\tildeh{\tilde{h}}
\def\tildei{\tilde{i}}
\def\tildej{\tilde{j}}
\def\tildek{\tilde{k}}
\def\tildel{\tilde{l}}
\def\tildem{\tilde{m}}
\def\tilden{\tilde{n}}
\def\tildeo{\tilde{o}}
\def\tildep{\tilde{p}}
\def\tildeq{\tilde{q}}
\def\tilder{\tilde{r}}
\def\tildes{\tilde{s}}
\def\tildet{\tilde{t}}
\def\tildeu{\tilde{u}}
\def\tildev{\tilde{v}}
\def\tildew{\tilde{w}}
\def\tildex{\tilde{x}}
\def\tildey{\tilde{y}}
\def\tildez{\tilde{z}}


\def\tildeA{\tilde{A}}
\def\tildeB{\tilde{B}}
\def\tildeC{\tilde{C}}
\def\tildeD{\tilde{D}}
\def\tildeE{\tilde{E}}
\def\tildeF{\tilde{F}}
\def\tildeG{\tilde{G}}
\def\tildeH{\tilde{H}}
\def\tildeI{\tilde{I}}
\def\tildeJ{\tilde{J}}
\def\tildeK{\tilde{K}}
\def\tildeL{\tilde{L}}
\def\tildeM{\tilde{M}}
\def\tildeN{\tilde{N}}
\def\tildeO{\tilde{O}}
\def\tildeP{\tilde{P}}
\def\tildeQ{\tilde{Q}}
\def\tildeR{\tilde{R}}
\def\tildeS{\tilde{S}}
\def\tildeT{\tilde{T}}
\def\tildeU{\tilde{U}}
\def\tildeV{\tilde{V}}
\def\tildeW{\tilde{W}}
\def\tildeX{\tilde{X}}
\def\tildeY{\tilde{Y}}
\def\tildeZ{\tilde{Z}}


\def\tildetheta{\tilde{\theta}}
\def\tildeDelta{\tilde{\Delta}}


%==========================
%==========================
%====Bold hat symbols =====
\def\boldhata{\hat{\boldsymbol{a}}}
\def\boldhatb{\hat{\boldsymbol{b}}}
\def\boldhatc{\hat{\boldsymbol{c}}}
\def\boldhatd{\hat{\boldsymbol{d}}}
\def\boldhate{\hat{\boldsymbol{e}}}
\def\boldhatf{\hat{\boldsymbol{f}}}
\def\boldhatg{\hat{\boldsymbol{g}}}
\def\boldhath{\hat{\boldsymbol{h}}}
\def\boldhati{\hat{\boldsymbol{i}}}
\def\boldhatj{\hat{\boldsymbol{j}}}
\def\boldhatk{\hat{\boldsymbol{k}}}
\def\boldhatl{\hat{\boldsymbol{l}}}
\def\boldhatm{\hat{\boldsymbol{m}}}
\def\boldhatn{\hat{\boldsymbol{n}}}
\def\boldhato{\hat{\boldsymbol{o}}}
\def\boldhatp{\hat{\boldsymbol{p}}}
\def\boldhatq{\hat{\boldsymbol{q}}}
\def\boldhatr{\hat{\boldsymbol{r}}}
\def\boldhats{\hat{\boldsymbol{s}}}
\def\boldhatt{\hat{\boldsymbol{t}}}
\def\boldhatu{\hat{\boldsymbol{u}}}
\def\boldhatv{\hat{\boldsymbol{v}}}
\def\boldhatw{\hat{\boldsymbol{w}}}
\def\boldhatx{\hat{\boldsymbol{x}}}
\def\boldhaty{\hat{\boldsymbol{y}}}
\def\boldhatz{\hat{\boldsymbol{z}}}

\def\boldhatA{\hat{\boldsymbol{A}}}
\def\boldhatB{\hat{\boldsymbol{B}}}
\def\boldhatC{\hat{\boldsymbol{C}}}
\def\boldhatD{\hat{\boldsymbol{D}}}
\def\boldhatE{\hat{\boldsymbol{E}}}
\def\boldhatF{\hat{\boldsymbol{F}}}
\def\boldhatG{\hat{\boldsymbol{G}}}
\def\boldhatH{\hat{\boldsymbol{H}}}
\def\boldhatI{\hat{\boldsymbol{I}}}
\def\boldhatJ{\hat{\boldsymbol{J}}}
\def\boldhatK{\hat{\boldsymbol{K}}}
\def\boldhatL{\hat{\boldsymbol{L}}}
\def\boldhatM{\hat{\boldsymbol{M}}}
\def\boldhatN{\hat{\boldsymbol{N}}}
\def\boldhatO{\hat{\boldsymbol{O}}}
\def\boldhatP{\hat{\boldsymbol{P}}}
\def\boldhatQ{\hat{\boldsymbol{Q}}}
\def\boldhatR{\hat{\boldsymbol{R}}}
\def\boldhatS{\hat{\boldsymbol{S}}}
\def\boldhatT{\hat{\boldsymbol{T}}}
\def\boldhatU{\hat{\boldsymbol{U}}}
\def\boldhatV{\hat{\boldsymbol{V}}}
\def\boldhatW{\hat{\boldsymbol{W}}}
\def\boldhatX{\hat{\boldsymbol{X}}}
\def\boldhatY{\hat{\boldsymbol{Y}}}
\def\boldhatZ{\hat{\boldsymbol{Z}}}




\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}

\newtheorem{thm}{Thm}
\newtheorem{defn}{Defn}
\newtheorem{ex}{Ex}
\newtheorem{prop}{Prop}
\newtheorem{rem}{Rem}
\newtheorem{lem}{Lem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\span{\mbox{span}}
\def\supp{\mbox{supp}}


\newcommand{\colBlue}[1]{\textcolor{blue}{#1}}
\newcommand{\colRed}[1]{\textcolor{red}{#1}}
\newcommand{\colMagenta}[1]{\textcolor{magenta}{#1}}
\newcommand{\colViolet}[1]{\textcolor{violet}{#1}}
\newcommand{\colGreen}[1]{\textcolor{darkgreen}{#1}}



==> sty/LatexPackages.tex <==
\usepackage[utf8]{inputenc}
\usepackage{stackengine}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathrsfs}
\usepackage{ulem}
\usepackage{epsf,epsfig}
\usepackage{cite}
\usepackage{color,xcolor}
\usepackage{dsfont}
\usepackage{bbm}
\usepackage{amsthm}
\usepackage{physics}
%\usepackage{undertilde}
\usepackage{tcolorbox}
\usepackage{wrapfig}
\usepackage{url}
\usepackage{graphicx}
% \usepackage{geometry}
% \usepackage{titling}
% \usepackage{hyperref}
\usepackage{eurosym}
\usepackage{enumitem}
\usepackage{nopageno}
\usepackage{fancyhdr}
\usepackage{mathtools}
\usepackage{stmaryrd}


